DiM: Distilling Dataset into Generative Model

Dataset distillation reduces the network training cost by synthesizing small and informative datasets from large-scale ones. Despite the success of the recent dataset distillation algorithms, three drawbacks still limit their wider application: i). the synthetic images perform poorly on large architectures; ii). they need to be re-optimized when the distillation ratio changes; iii). the limited diversity restricts the performance when the distillation ratio is large. In this paper, we propose a novel distillation scheme to \textbf{D}istill information of large train sets \textbf{i}nto generative \textbf{M}odels, named DiM. Specifically, DiM learns to use a generative model to store the information of the target dataset. During the distillation phase, we minimize the differences in logits predicted by a models pool between real and generated images. At the deployment stage, the generative model synthesizes various training samples from random noises on the fly. Due to the simple yet effective designs, the trained DiM can be directly applied to different distillation ratios and large architectures without extra cost. We validate the proposed DiM across 4 datasets and achieve state-of-the-art results on all of them. To the best of our knowledge, we are the first to achieve higher accuracy on complex architectures than simple ones, such as 75.1\% with ResNet-18 and 72.6\% with ConvNet-3 on ten images per class of CIFAR-10. Besides, DiM outperforms previous methods with 10\% $\sim$ 22\% when images per class are 1 and 10 on the SVHN dataset.

==> tabs/abl_B.tex <==
\begin{table}[h]
    \centering
    \small
    \begin{tabular}{c|c|c|c|c|c|c}
        \toprule
        Acc. /$\mathbf{B}$ & 16 & 32 & 64 & 128 & 256 & 384 \\
        \midrule
        C-3 &69.97  &71.76  &72.63 &72.39 &72.37 &71.93 \\
        % R-10 &  &  &73.55 &73.08 &69.51 &70.11 & \\
        \bottomrule
    \end{tabular}
    \caption{Ablation of $\mathbf{B}$. The best result is marked in \textbf{bold}.}
    \label{tab:abl_B}
\end{table}
